Iniva: Inclusive and Incentive-compatible Vote Aggregation

Many blockchain platforms use committee-based consensus for scalability, finality, and security. In this consensus scheme, a committee decides which blocks get appended to the chain, typically through several voting phases. Platforms typically leverage the committee members' recorded votes to reward, punish, or detect failures. A common approach is to let the block proposer decide which votes to include, opening the door to possible attacks. For example, a malicious proposer can omit votes from targeted committee members, resulting in lost profits and, ultimately, their departure from the system. This paper presents Iniva, an inclusive and incentive-compatible vote aggregation scheme that prevents such vote omission attacks. Iniva relies on a tree overlay with carefully selected fallback paths, making it robust against process failures without needing reconfiguration or additional redundancy. Our analysis shows that Iniva significantly reduces the chance to omit individual votes while ensuring that omitting many votes incurs a significant cost. In addition, our experimental results show that Iniva enjoys robustness, scalability, and reasonable throughput.

==> plots/figures/base_plot.tex <==
%\begin{figure*}[h]
%
%    \centering
%    \begin{subfigure}[b]{0.49\textwidth}
%        \centering
%        \resizebox{\linewidth}{!}{%
%        \input{plots/baseval2.tex}
%        }
%        \caption{Throughput vs Latency plot for HotStuff, \proj with sending \scndchance, and \proj without sending \scndchance. }
%        \label{fig: baseperf}
%    \end{subfigure} \hfill
%    \begin{subfigure}[b]{0.49\textwidth}
%        \centering
%        \resizebox{\linewidth}{!}{%
%        \input{plots/cpubls12.tex}
%        }
%        \caption{CPU usage of HotStuff and \proj.  }
 %       \label{fig:bls12cpu}
%    \end{subfigure}
%    \caption{Base evaluation experiment. The experiment is run using 21 replicas with 4 clients. The experiment is repeated with 100 and 800 batch sizes and 64 and 128 payloads. Bls12 is used for aggregating the signatures.}
%    \label{fig:base_experiments}
%\end{figure*}


\begin{figure}[!ht]
    \centering
        \resizebox{\linewidth}{!}{%
        \input{plots/baseval2.tex}
        }
       \caption{Base evaluation experiment for throughput vs Latency plot for HotStuff, \proj with sending \scndchance, and \proj without sending \scndchance. %The experiment is run using 21 replicas with 4 clients. The experiment is repeated with 100 and 800 batch sizes and 64 and 128 payloads. Bls12 is used for aggregating the signatures.
       }
\label{fig:baseperf}
\end{figure}

\begin{figure}[!ht]
    \centering
        \resizebox{\linewidth}{!}{%
        \input{plots/cpubls12.tex}
        }
       \caption{CPU usage of HotStuff and \proj. %The experiment is run using 21 replicas with 4 clients. The experiment is repeated with 100 and 800 batch sizes and 64 and 128 payloads. Bls12 is used for aggregating the signatures.
       }
\label{fig:bls12cpu}
\end{figure}


==> plots/figures/scale_plot.tex <==
\begin{figure}[!ht]
    \centering
        \resizebox{\linewidth}{!}{%
        \input{plots/config_th.tex}
        }
       \caption{Scalability evaluation with batchsize B=100 and 
varying configuration sizes and payloads.
    %5 replicas on each node for 
Configuration sizes are selected to have an almost complete tree of height 3.}
\label{fig:configlth}
\end{figure}

%\begin{figure*}[h]
%     \begin{subfigure}[b]{0.49\textwidth}
%        \centering
%        \resizebox{\linewidth}{!}{%
%        \input{plots/config_th.tex}
%        }
%        \caption{Throughput. } 
%        \label{fig:configlth}
%    \end{subfigure} \hfill
%    \begin{subfigure}[b]{0.49\textwidth}
%        \centering
%        \resizebox{\linewidth}{!}{%
%        \input{plots/config_lt.tex}
%        }
%        \caption{Latency.} 
%        \label{fig:configlt}
%        \end{subfigure}
    
%    \caption{Scalability evaluation with batchsize B=100 and 
%varying configuration sizes and payloads.
    %5 replicas on each node for 
%Configuration sizes are selected to have an almost complete tree of height 3.}
%    \label{fig:scale_experiments}
%\end{figure*}

